Hierarchical Clustering better than Average-Linkage

Hierarchical Clustering (HC) is a widely studied problem in exploratory data analysis, usually tackled by simple agglomerative procedures like average-linkage, single-linkage or complete-linkage. In this paper we focus on two objectives, introduced recently to give insight into the performance of average-linkage clustering: a similarity based HC objective proposed by [Moseley and Wang, 2017] and a dissimilarity based HC objective proposed by [Cohen-Addad et al., 2018]. In both cases, we present tight counterexamples showing that average-linkage cannot obtain better than 1/3 and 2/3 approximations respectively (in the worst-case), settling an open question raised in [Moseley and Wang, 2017]. This matches the approximation ratio of a random solution, raising a natural question: can we beat average-linkage for these objectives? We answer this in the affirmative, giving two new algorithms based on semidefinite programming with provably better guarantees.

==> notations.tex <==
\newcommand{\nonleaf}[1]{\textbf{non-leaves}(#1)}
\newcommand{\xijt}[1]{x^{(#1)}_{ij}}
\newcommand{\vit}[2]{\mathbf{v}^{(#2)}_{#1}}
\newcommand{\norms}[1]{\lVert #1 \rVert_2^2}

For any given clustering tree $T$, let $i\vee j$ denotes the least common ancestor of the two data points $i$ and $j$ in $T$. Let $T[u]$ denote the subtree of $T$ that is rooted at cluster $u$, and $\nonleaf{T'}$ denote the set of all data points that are \emph{not} a leaf of the subtree $T'\subseteq T$.  

We consider a variant of the \emph{Hierarchical Clustering} (HC) problem, where the goal is find a clustering tree $T$ given the weights $\{w_{ij}\}$ that minimizes the following objective function:
\begin{equation}
\sum_{(i,j)\in E}w_{ij}\lvert\nonleaf{T[i \vee j]}\rvert
\end{equation}

Suppose we have $n$ data points. An alternative view of a hierarchical clustering of these points is a collection of partitioning of the points at different levels $t=n-1,\ldots,1$, where the partitions at level $t$ are all maximal clusters of size at most $t$. Given this view, one can rewrite the above objective function of the clustering problem as following:
\begin{equation}
\sum_{t=1}^{n-1}\sum_{(i,j)\in E}w_{i,j}\cdot \mathbf{1}\{\textrm{$i$ and $j$ are not separated at level $t$'s partitioning}\}
\end{equation}
Given this alternative view, one can write the following SDP relaxation for the hierarchical clustering problem.
\begin{proposition}
The following semi-definite program is a relaxation for the HC problem.
\begin{equation}
\label{eq:SDP-HC}
\begin{aligned}
& \underset{}{\text{maximize}}
& & \sum_{t=1}^{n-1}\sum_{(i,j)\in E}w_{ij}(1-\xijt{t}) \\
& \text{subject to}
& & \xijt{t}=\frac{1}{2}\norms{\vit{i}{t}-\vit{j}{t}}, & \forall(i,j) \in E, t\in[1:n-1]\\
& 
& & \sum_{j}\xijt{t}\geq n-t, & \forall (i,j)\in E,t\in[1:n-1]\\
&
& & \xijt{t+1}\leq \xijt{t}& \forall(i,j)\in E,t\in[1:n-1]\\
&
& & \vit{i}{t}\in\mathbb{R}^n,~~\norms{\vit{i}{t}}=1, & \forall i\in V,t\in[1:n-1]
\end{aligned}
\end{equation}
\end{proposition}


==> sdp-dissimilarity.tex <==
\subsection{Warm-up: SDP Rounding of the First Cut}
We consider two simple algorithms for the HC problem. The first algorithm, \emph{Random-Always}, cuts each cluster recursively and uniformly at random until it reaches to singletons. The second algorithm, \emph{SDP-First-Random-Next}, uses SDP and rounding for determining the first cut, and then picks a random cut after for each of the later clusters until it reaches to singletons. 

\begin{algorithm}[h]
\caption{Random-Always}
\label{alg:Random}
\begin{algorithmic}[1]
\State \textbf{input}: $G=(V,E)$.
\If {$\lvert V \rvert=1$} 
\State Return the singleton vertex as the only cluster.
\Else
\State Randomly partition the set of vertices into $S$ and $\bar{S}$. 
\State Recursively run \emph{Random-Always} on $G_S$ and $G_{\bar{S}}$ to get clusters $\mathcal{C}_S$ and $\mathcal{C}_{\bar{S}}$.
\State Return the clusters $S$,$\bar{S}$, $\mathcal{C}_S$ and $\mathcal{C}_{\bar{S}}$. 
\EndIf
\end{algorithmic}
\end{algorithm}
\begin{algorithm}[h]
\caption{SDP-First-Random-Next}
\label{alg:SDP-Random}
\begin{algorithmic}[1]
\State \textbf{input:} $G=(V,E)$ and weights $\{w_{ij}\}_{(i,j)\in E}$.
\State Solve the SDP of HC (as in Proposition~\ref{eq:SDP-HC}). 
\State Let $x^*_{ij}=\xijt{\floor{(n-1)/2}}$ and $\mathbf{v}^*_i=\vit{i}{\floor{(n-1)/2}}$ be the optimal solution restricted to level $t=\floor{(n-1)/2}$.
\State Draw $\mathbf{v}_0$ uniformly at random from unit sphere, and let $S=\{i\in V: \mathbf{v}^*_i\cdot \mathbf{v}_0\geq 0\}$.
\State Partition the vertices into $S$ and $\bar{S}=V\setminus S$. 
\State Run \emph{Random-Always} (Algorithm~\ref{alg:Random}) on $S$ and $\bar{S}$ to get clusters $\mathcal{C}_S$ and $\mathcal{C}_{\bar{S}}$.
\State Return the clusters $S$,$\bar{S}$, $\mathcal{C}_S$ and $\mathcal{C}_{\bar{S}}$. 
\end{algorithmic}
\end{algorithm}
\begin{theorem}
The algorithm that outputs the best of \emph{SDP-First-Random-Next} (Algorithm~\ref{alg:SDP-Random}) and \emph{Random-Always} (Algorithm~\ref{alg:Random}) is a randomized $(\frac{8}{9(1+\sqrt{\frac{11+2\pi}{3+2\pi}})})$-approximation for the HC problem.
\end{theorem}
\begin{proof}
We start by looking at the objective value of any algorithm as the summation of contributions of different triplets $i,j$ and $k$ to the objective, where $(i,j)\in E$ and $k\neq i,j$ is some other vertex. 
\begin{equation}
\OBJ=\sum_{(i,j)\in E}w_{ij}\lvert\nonleaf{T[i \vee j]}\rvert=\sum_{(i,j)\in E}\sum_{k\neq i,j}w_{ij}\mathbf{1}\{\textrm{$k$ is a non-leaf of $T[i\vee j]$}\}
\end{equation}
The vertex $k$ is a non-leaf vertex of $T[i\vee j]$ if and only if at some point during the execution of the algorithm $k$ gets separated from $i$ and $j$, while $i$ and $j$ still remain in the same cluster. Let random variables $\Zcal_{i,j,k}$ and $\Ycal_{i,j,k}$ denote the contributions of the edge $(i,j)$ and vertex $k\neq i,j$ to the objective value of Algorithm~\ref{alg:Random} and Algorithm~\ref{alg:SDP-Random} respectively, i.e. 
$$\Zcal_{i,j,k}\triangleq w_{ij}\mathbf{1}\{\textrm{$k$ is a non-leaf of $T_{\textrm{ALG}_1}[i\vee j]$}\}~~~\textrm{and}~~~ \Ycal_{i,j,k}\triangleq w_{ij}\mathbf{1}\{\textrm{$k$ is a non-leaf of $T_{\textrm{ALG}_2}[i\vee j]$}\}$$
Moreover, let $\Ycal_{i,j}=\sum_{k\neq i,j}\Ycal_{i,j,k}$ and $\Zcal_{i,j}=\sum_{k\neq i,j}\Zcal_{i,j,k}$. Let $\OPT$ be the optimal value of the HC objective. Fix $\epsilon_1>0$ and consider two cases. 

\paragraph{\textbf{Case 1:}}  $\OPT < (1-\epsilon_1)(n-1)\Ws$. A simple argument shows that $\Ex{\Zcal_{i,j,k}}=\frac{1}{3}w_{ij}$. Given this, the expected objective value of  Algorithm~\ref{alg:Random} will be at least $\frac{n-2}{3}\sum_{(i,j)\in E}w_{ij}$, and hence Algorithm~\ref{alg:Random} achieves $\frac{n-2}{n-1}\cdot\frac{1}{3(1-\epsilon_1)}$ fraction of $\OPT$ in this case. To see this why this holds, think of randomized cutting as flipping an independent unbiased coin for each vertex, and then deciding on which side of the cut this vertex belongs to based on the outcome of its coin. Look at the sequence of the coin flips of $i$, $j$ and $k$. Our goal is to find the probability of the event that for the first time these three sequences are not matched, but $i$'s sequence and $j$'s sequence are still matched. Fixing $i$'s sequence, the probability that all three are always matched is $\sum_{i=1}^{\infty}(1/4)^i=1/3$. Due to the symmetry, the rest of the probability will be divided equally between our target event and the event that for the first time these three sequences are not matched, but still $i$'s sequence and $k$'s sequence are matched. Therefore, $\Pr{\textrm{$k$ is a non-leaf of $T_{\textrm{ALG}_1}[i\vee j]$}}=1/3$, which proves what we desired. 


\paragraph{\textbf{Case 2:}}  $\OPT \geq (n-1)(1-\epsilon_1)\Ws$. In this case, our goal is to bound the objective value of Algorithm~\ref{alg:SDP-Random}. To this end, we show how to bound $\Ex{\Ycal_{i,j}}$. Consider the following events:
\begin{align*}
\Ecal_{i,j}&\triangleq \{\textrm{$i$ and $j$ remain together after the first cut}\},\\
\Ecal_{i,j,k}&\triangleq \{\textrm{$i$, $j$ and $k$  remain together after the first cut}\},\\
\bar{\Ecal}_{i,j,k}&\triangleq \{\textrm{$i$, $j$ remain together and $k$  gets separated after the first cut}\}
\end{align*}
 We can rewrite $\Ex{\Ycal_{i,j,k}}$ as follows.
\begin{align*}
\Ex{\Ycal_{i,j,k}}&=\Ex{\Ycal_{i,j,k}|\Ecal_{i,j}}\Pr{\Ecal_{i,j}}=\left(\Ex{\Ycal_{i,j,k}\mathbf{1}\{\Ecal_{i,j,k}\}|\Ecal_{i,j}}+\Ex{\Ycal_{i,j,k}\mathbf{1}\{\bar{\Ecal}_{i,j,k}\}|\Ecal_{i,j}}\right)\Pr{\Ecal_{i,j}}\\
&=\left(\Ex{\Ycal_{i,j,k}|\Ecal_{i,j,k}}\Pr{\Ecal_{i,j,k}|\Ecal_{i,j}}+\Ex{\Ycal_{i,j,k}|\bar{\Ecal}_{i,j,k}}\Pr{\bar{\Ecal}_{i,j,k}|\Ecal_{i,j}}\right)\Pr{\Ecal_{i,j}}
\end{align*}
Now, note that $\Ex{\Ycal_{i,j,k}|\bar{\Ecal}_{i,j,k}}=w_{ij}$, as $k$ has been separated from $i$ and $j$ after the first cut.  Moreover, $\Pr{\textrm{$k$ is a non-leaf of $T_{\textrm{ALG}_2}[i\vee j]$}|\Ecal_{i,j,k}}=1/3$, as Algorithm~\ref{alg:SDP-Random} performs random cuts after the first cut and the previous argument for analyzing $\Zcal_{i,j,k}$ will be applied. So, $\Ex{\Ycal_{i,j,k}|\Ecal_{i,j,k}}=w_{ij}/3$. Therefore, we have the following:
\begin{align*}
\Ex{\Ycal_{i,j,k}}&=\left(\frac{w_{ij}}{3}\Pr{\Ecal_{i,j,k}|\Ecal_{i,j}}+w_{ij}\Pr{\bar{\Ecal}_{i,j,k}|\Ecal_{i,j}}\right)\Pr{\Ecal_{i,j}}=w_{ij}\Pr{\Ecal_{i,j}}\left(\frac{1}{3}+\frac{2}{3}\Pr{\bar{\Ecal}_{i,j,k}|\Ecal_{i,j}}\right),
\end{align*}
and hence we have
\begin{equation}
\label{eq:yijk}
\Ex{\Ycal_{i,j}}=\sum_{k\neq i,j}\Ex{\Ycal_{i,j,k}}=w_{ij}\left(\Pr{\Ecal_{i,j}}\frac{n-2}{3}+\frac{2}{3}\sum_{k\neq i,j}\Pr{\bar{\Ecal}_{i,j,k}}\right)
\end{equation}
Fix $\epsilon_2>0$ and consider all edges for which $x^*_{ij}=\xijt{\floor{(n-1)/2}}\leq \epsilon_2$ (denoted by $\mathcal{H}\subseteq E$).  For every such edge $(i,j)$, by applying the basics of hyperplane rounding, we have:
\begin{equation*}
\Pr{\Ecal_{i,j}}=\Pr{(\mathbf{v}^*_i\cdot \mathbf{v}_0)(\mathbf{v}^*_j\cdot \mathbf{v}_0)\geq 0}=1-\theta_{i,j}/\pi,
\end{equation*}
where $\theta_{i,j}$ is defined to be the angel between the vectors $\mathbf{v}^*_i$ and $\mathbf{v}^*_j$, i.e. $\theta_{i,j}=\cos^{-1}(\mathbf{v}^*_i\cdot\mathbf{v}^*_j)=\cos^{-1}(1-x^*_{ij})$. Now, it is clear that $\theta_{i,j}\leq \bar{\theta}$, where $1-\cos(\bar{\theta})=\epsilon_2$, for edges in $\mathcal{H}$. Therefore,
\begin{equation}
\label{eq:h-lower}
\Pr{\Ecal_{i,j}}\geq 1-\bar{\theta}/\pi,~~~\forall (i,j)\in \mathcal{H}
\end{equation}
We now bound $\sum_{k\neq i,j}\Pr{\bar{\Ecal}_{i,j,k}}$ for every edge $(i,j)\in\mathcal{H}$. Define $\theta^{(k)}\in[0,\pi]$ to be the angel between $\mathbf{v}^*_k$ and $\mathbf{v}^*_i$. Again, by applying a basic argument from hyperplane rounding,  $\Pr{\bar{\Ecal}_{i,j,k}}=\max(\frac{\theta^{(k)}}{\pi}-\frac{\bar{\theta}}{\pi},0)$. Note that due to the spreading constraint in the SDP, we have $\sum_{k\neq i}{x^*_{ik}}\geq n-\floor{(n-1)/2}$, and therefore $\sum_{k\neq i}\cos(\theta^{(k)})\leq (n-1)/2$. So, one can bound $\sum_{k\neq i,j}\Pr{\bar{\Ecal}_{i,j,k}}$ by the optimal solution of the following optimization problem:
\begin{equation*}
\begin{aligned}
& \underset{}{\text{minimize}}
& & \sum_{k\neq i} (\frac{\theta^{(k)}}{\pi}-\frac{\bar{\theta}}{\pi}) \\
& \text{subject to}
& & \sum_{k\neq i}\cos(\theta^{(k)})\leq (n-1)/2, & \\
& 
& & \theta^{(k)}\geq \bar{\theta}, &~~~\forall k\neq i\\
\end{aligned}
\end{equation*}
Because of a simple symmetry argument, the optimal solution to the above program is achieved at a symmetric solution. If $\epsilon_2\leq 1/2$, then $\bar{\theta}\leq \pi/3$, and in this case the optimal solution would be $\theta^{(k)}=\pi/3$. Therefore, we conclude the following lowerbound if $\epsilon_2\leq \frac{1}{2}$:
\begin{equation}
\label{eq:spreading-OPT}
\sum_{k\neq i,j}\Pr{\bar{\Ecal}_{i,j,k}}\geq (n-1)(\frac{1}{3}-\frac{\bar{\theta}}{\pi})
\end{equation}  

By putting (\ref{eq:yijk}), (\ref{eq:h-lower}) and (\ref{eq:spreading-OPT}) together, we have:
\begin{equation*}
\Ex{\OBJ_{\textrm{ALG}_2}}\geq \sum_{(i,j)\in\mathcal{H}}\Ex{\Ycal_{i,j}}\geq (n-2)\left(\frac{5}{9}-\frac{\bar{\theta}}{\pi} \right)\sum_{(i,j)\in\mathcal{H}}w_{ij}
\end{equation*}
We finally bound the total weight of edges in $\mathcal{H}$. Note that for an edge $(i,j)\notin\mathcal{H}$, $\xijt{t}>\epsilon_2,\forall 1\leq t\leq \floor{n/2}$, due to the monotonicity constrain in SDP. Now we have the following:
\begin{align*}
\textrm{\SDP}&=\sum_{t=1}^{n-1}\sum_{(i,j)\in E}w_{ij}(1-\xijt{t})\leq(n-1)\sum_{(i,j)\in E}w_{ij}-\sum_{t=1}^{\floor{(n-1)/2}}\sum_{(i,j)\in E}w_{ij}\xijt{t}\\
& \leq (n-1)\sum_{(i,j)\in E}w_{ij}-\frac{\epsilon_2(n-1)}{2}\cdot\sum_{(i,j)\in E\setminus \mathcal{H}}w_{ij}
\end{align*}
On the other hand, based on the assumption of Case 2, we know 
\begin{equation}
\SDP\geq\OPT\geq (n-1)(1-\epsilon_1)\sum_{(i,j)\in E}w_{ij}
\end{equation}
and therefore by rearranging the terms we have $\sum_{(i,j)\in \mathcal{H}}w_{ij}\geq (1-\frac{2\epsilon_1}{\epsilon_2})\Ws$, which shows Algorithm~\ref{alg:SDP-Random} achieves $\frac{n-2}{n-1}(1-\frac{2\epsilon_1}{\epsilon_2})(\frac{5}{9}-\frac{\cos^{-1}(1-\epsilon_2)}{\pi})$ fraction of $\OPT$. 

By balancing out the two cases, we have:
\begin{equation}
(1-\frac{2\epsilon_1}{\epsilon_2})(\frac{5}{9}-\frac{\cos^{-1}(1-\epsilon_2)}{\pi})=\frac{1}{3(1-\epsilon_1)}
\end{equation}

\end{proof}

